Rademacher Random Projections with Tensor Networks

Random projection (RP) have recently emerged as popular techniques in the machine learning community for their ability in reducing the dimension of very high-dimensional tensors. Following the work in [30], we consider a tensorized random projection relying on Tensor Train (TT) decomposition where each element of the core tensors is drawn from a Rademacher distribution. Our theoretical results reveal that the Gaussian low-rank tensor represented in compressed form in TT format in [30] can be replaced by a TT tensor with core elements drawn from a Rademacher distribution with the same embedding size. Experiments on synthetic data demonstrate that tensorized Rademacher RP can outperform the tensorized Gaussian RP studied in [30]. In addition, we show both theoretically and experimentally, that the tensorized RP in the Matrix Product Operator (MPO) format is not a Johnson-Lindenstrauss transform (JLT) and therefore not a well-suited random projection map

==> TN_proof.tex <==
\begin{center}
\scalebox{1}{{\parbox{.5\linewidth}{
\begin{align*}
    \EE[\nbr{\yb}_2^2] 
&=
    \EE\left[
    \begin{tikzpicture}[baseline=0.5ex]
    \tikzset{tensor/.style = {minimum size = 0.6cm,shape = circle,thick,draw=black,inner sep = 0pt}, edge/.style   = {thick,line width=.4mm},every loop/.style={}}
    \def\y{0}
    \def\x{0}
    \def\inc{2}
    \node[tensor,fill=red!50!white] (G1) at (\x,\y+1/2) {\scalebox{0.85}{$\Gt^1$}};
    \node[tensor,fill=blue!40!red!60!white] (G2) at (\x+\inc,\y+1/2) {\scalebox{0.85}{$ \Gt^{2}$}};
    \node[tensor,fill=blue!40!white] (X) at (\x+1,\y-1/4) {\scalebox{0.85}{$\Xb$}};
    \node[tensor,fill=blue!40!red!60!white] (G2prime) at (\x+2*\inc,\y+1/2) {\scalebox{0.85}{$ \Gt^{2}$}};
    \node[tensor,fill=red!50!white] (G1prime) at (\x+3*\inc,\y+1/2) {\scalebox{0.85}{$\Gt^1$}};
    \node[tensor,fill=blue!40!white] (Xprime) at (\x+5,\y-1/4) {\scalebox{0.85}{$\Xb$}};
    \draw[edge] (G1) -- (G2)node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$R$}}};
    \draw[edge] (G2) -- (G2prime) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$k$}}};
    \draw[edge] (G2prime) -- (G1prime) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$R$}}};
    \draw[edge] (G2prime) -- (Xprime) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
    \draw[edge] (G1prime) -- (Xprime) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
    \draw[edge] (G1) -- (X) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
    \draw[edge] (G2) -- (X) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
    \end{tikzpicture}
    \right]\\
%
%
&=
%
%
\EE\Bigg[
\begin{tikzpicture}[baseline=0.5ex]
\tikzset{tensor/.style = {minimum size = 0.6cm,shape = circle,thick,draw=black,inner sep = 0pt}, edge/.style   = {thick,line width=.4mm},every loop/.style={}}
\def\y{0}
\def\x{0}
\def\inc{2}
\node[tensor,fill=red!50!white] (G1) at (\x,\y+1/2) {\scalebox{0.85}{$\Gt^1$}};
\node[tensor,fill=red!50!white] (G1prime) at (\x+1,\y+1/2) {\scalebox{0.85}{$\Gt^1$}};
\draw[edge] (\x+.3,\y+1/2) -- (\x+.3,\y-1/4)  node [right] {\scalebox{0.6}{\textcolor{gray}{$R$}}};
\draw[edge] (\x-.3,\y+1/2) -- (\x-.3,\y-1/4)  node [left] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (\x+1.3,\y+1/2) -- (\x+1.3,\y-1/4)  node [right] {\scalebox{0.6}{\textcolor{gray}{$R$}}};
\draw[edge] (\x+0.7,\y+1/2) -- (\x+0.7,\y-1/4)  node [right] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\end{tikzpicture}
\Bigg]
\EE\Bigg[
\begin{tikzpicture}[baseline=0.5ex]
\tikzset{tensor/.style = {minimum size = 0.6cm,shape = circle,thick,draw=black,inner sep = 0pt}, edge/.style   = {thick,line width=.4mm},every loop/.style={}}
\def\y{0}
\def\x{0}
\def\inc{2}
\node[tensor,fill=blue!40!white] (X) at (\x-1,\y+1/4){\scalebox{0.85}{$ \Xb$}};
\node[tensor,fill=blue!40!red!60!white] (G2) at (\x,\y+1/4) {\scalebox{0.85}{$ \Gt^{2}$}};
\node[tensor,fill=blue!40!red!60!white] (G2prime) at (\x+1,\y+1/4) {\scalebox{0.85}{$ \Gt^{2}$}};
\node[tensor,fill=blue!40!white] (Xprime) at (\x+2,\y+1/4) {\scalebox{0.85}{$\Xb$}};
\draw[edge] (G2) -- (G2prime) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$k$}}};
\draw[edge] (G2prime) -- (Xprime) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (X) -- (G2) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (Xprime) to[out=-135,in=-45, distance=0.7cm] (X) node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (G2) to[out=90,in=90] (G2prime) node [above,midway]{\scalebox{0.6}{\textcolor{gray}{$d$}}};
\end{tikzpicture}
\Bigg]\\
&= 
\Ib_{Rd}
\left(\EE\Bigg[
\begin{tikzpicture}[baseline=0.5ex]
\tikzset{tensor/.style = {minimum size = 0.6cm,shape = circle,thick,draw=black,inner sep = 0pt}, edge/.style   = {thick,line width=.4mm},every loop/.style={}}
\def\y{0}
\def\x{0}
\node[tensor,fill=blue!40!red!60!white] (G2) at (\x,\y+1/2) {\scalebox{0.85}{$\Gt^2$}};
\node[tensor,fill=blue!40!red!60!white] (G2prime) at (\x+1,\y+1/2) {\scalebox{0.85}{$\Gt^2$}};
\draw[edge] (\x+.27,\y+0.6) -- (\x+.73,\y+0.6)  node [above,midway] {\scalebox{0.6}{\textcolor{gray}{$R$}}};
\draw[edge] (\x-.3,\y+1/2) -- (\x-.3,\y-1/4)  node [left] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (\x+1.3,\y+1/2) -- (\x+1.3,\y-1/4)  node [right] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (\x+0.27,\y+0.4) -- (\x+0.73,\y+0.4)  node [below,midway] {\scalebox{0.6}{\textcolor{gray}{$k$}}};
\end{tikzpicture}
\Bigg]
\EE\Bigg[
\begin{tikzpicture}[baseline=0.5ex]
\tikzset{tensor/.style = {minimum size = 0.6cm,shape = circle,thick,draw=black,inner sep = 0pt}, edge/.style   = {thick,line width=.4mm},every loop/.style={}}
\def\y{0}
\def\x{0}
\node[tensor,fill=blue!40!white] (X) at (\x,\y+1/2){\scalebox{0.85}{$ \Xb$}};
\node[tensor,fill=blue!40!white] (Xprime) at (\x+1,\y+1/2){\scalebox{0.85}{$ \Xb$}};
\draw[edge] (X) -- (Xprime) node [above,midway]
{\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (\x-.3,\y+1/2) -- (\x-.3,\y-1/4)  node [left] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\draw[edge] (\x+1.3,\y+1/2) -- (\x+1.3,\y-1/4)  node [right] {\scalebox{0.6}{\textcolor{gray}{$d$}}};
\end{tikzpicture}
\Bigg]\right)\\
&=
\EE\left[\vcenter{\hbox{\includegraphics[height=1.5cm]{./figures/TN-1.png}}}\right]
\end{align*}}}}
\end{center}
